An Effective and Differentially Private Protocol for Secure Distributed Cardinality Estimation

Counting the number of distinct elements distributed over multiple data holders is a fundamental problem with many real-world applications ranging from crowd counting to network monitoring. Although a number of space and computational efficient sketch methods (e.g., the Flajolet-Martin sketch and the HyperLogLog sketch) for cardinality estimation have been proposed to solve the above problem, these sketch methods are insecure when considering privacy concerns related to the use of each data holder's personal dataset. Despite a recently proposed protocol that successfully implements the well-known Flajolet-Martin (FM) sketch on a secret-sharing based multiparty computation (MPC) framework for solving the problem of private distributed cardinality estimation (PDCE), we observe that this MPC-FM protocol is not differentially private. In addition, the MPC-FM protocol is computationally expensive, which limits its applications to data holders with limited computation resources. To address the above issues, in this paper we propose a novel protocol DP-DICE, which is computationally efficient and differentially private for solving the problem of PDCE. Experimental results show that our DP-DICE achieves orders of magnitude speedup and reduces the estimation error by several times in comparison with state-of-the-arts under the same security requirements.

==> table_notations.tex <==
\pdfoutput=1
\begin{table}[t]
\begin{center}
\caption{Table of notations.\label{tab:notations}}
\begin{tabular}{|c|l|} \hline
%$\Pi$&graph stream of interest\\ \hline
$d$&the number of data holders (DHs)\\ \hline
$c$&the number of computing parties (CPs) \\ \hline
$S_j$&the set held by DH $j\in \{1, \ldots, d\}$\\ \hline
$U$&the universal set\\ \hline
$S$&the union of all sets $S_1, \ldots, S_d$\\ \hline
$n$&the number of elements in the union set $S$\\ \hline
$\hat n$& an estimate of cardinality $n$\\ \hline
$\{B_i^{(j)}\}_{i=1, \ldots, m}$&FMS sketch of set $S_j$\\\hline
$\{B_i\}_{i=1, \ldots, m}$&FMS sketch of the union set $S$\\\hline
$m=2^r$&the number of bit arrays used by our FMS\\ \hline
$w$&the size of each one-dimensional bit array $B_j$\\ \hline
$Z$&the number of zero bits in all arrays $B_1, \ldots, B_m$\\ \hline
$V$&the fraction of zero bits in all arrays $B_1, \ldots, B_m$\\ \hline
$N_j$&discrete noise generated by DH $j\in \{1, \ldots, d\}$\\ \hline
$N$& $N=\sum_{j=1}^d N_j$ is the total additive noise for $Z$\\ \hline
$p$&the modulus used for the SPDZ framework\\\hline
$L$&$L=\lceil \log_2 p\rceil$ is the bit length of $p$\\\hline
$\mathbb{F}_p$&$\mathbb{F}_p=\{0, 1, \ldots, p-1\}$\\\hline
\multirow{2}{*}{$h(e)$}&hash function that randomly maps an element\\
&$e\in U$ into a $(r+w-1)$-bit string\\\hline
$h^{(\text{L})}(e)$&the lowest $r$ bits of string $h(e)$\\\hline
$h^{(\text{H})}(e)$&the highest $w-1$ bits of string $h(e)$\\\hline
$\rho(h^{(\text{H})}(e))$ & the number of trailing zeros of $h^{(\text{H})}(e)$\\ \hline
$p_x$&the probability that $\rho\left(h^{(\text{H})}(e)\right)$ equals $x$\\ \hline
$\tau$&the bit length of the input plaintext for SPDZ\\\hline
$f(n)$&function defined as $f(n)= \frac{1}{w}\sum_{x=0}^{w-1} (1-p_x)^n$\\ \hline
$g(V)$&the inverse function of function $f(n)$\\\hline
$\llbracket{x}\rrbracket$&the shared form of an integer $x$ in SPDZ\\\hline
$\llbracket{x}\rrbracket_j$&secret share held by CP $j$\\\hline
$\varepsilon$&parameter for differential privacy\\\hline
$\varepsilon_d$&parameter for concentrated differential privacy\\\hline
\end{tabular}
\end{center}
\end{table}

